When Light Bends to the Collective Will: A Theory and Vision for Adaptive Photonic Scale-up Domains

As chip-to-chip silicon photonics gain traction for their bandwidth and energy efficiency, collective communication has emerged as a critical bottleneck in scale-up systems. Programmable photonic interconnects offer a promising path forward: by dynamically reconfiguring the fabric, they can establish direct, high-bandwidth optical paths between communicating endpoints -- \emph{synchronously and guided by the structure of collective operations} (e.g., AllReduce). However, realizing this vision -- \emph{when light bends to the collective will} -- requires navigating a fundamental trade-off between reconfiguration delay and the performance gains of adaptive topologies. In this paper, we present a simple theoretical framework for adaptive photonic scale-up domains that makes this trade-off explicit and clarifies when reconfiguration is worthwhile. Along the way, we highlight a connection -- not surprising but still powerful -- between the Birkhoff--von Neumann (BvN) decomposition, maximum concurrent flow (a classic measure of network throughput), and the well-known $\alpha$-$\beta$ cost model for collectives. Finally, we outline a research agenda in algorithm design and systems integration that can build on this foundation.

==> macros.tex <==
%!TEX ROOT = main.tex
\usepackage{enumitem}

\makeatletter
 \renewcommand\subsubsection{\@startsection {subsubsection}{3}{\z@}%
     {-2.5ex \@plus -1ex \@minus -.2ex}%
     {1.3ex \@plus.2ex}%
    {\ACM@NRadjust\@subsubsecfont}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%     {-.75\baselineskip \@plus -.2\p@ \@minus -.2\p@}% before \@plus -2\p@ <<<
%     {.25\baselineskip}%
%     {\ACM@NRadjust\@secfont}}
% \@startsection {NAME}{LEVEL}{INDENT}{BEFORESKIP}{AFTERSKIP}{STYLE} 
%            optional * [ALTHEADING]{HEADING}
%    Generic command to start a section.  
%    NAME       : e.g., 'subsection'
%    LEVEL      : a number, denoting depth of section -- e.g., chapter=1,
%                 section = 2, etc.  A section number will be printed if
%                 and only if LEVEL gt or eq the value of the secnumdepth
%                 counter.
%    INDENT     : Indentation of heading from left margin
%    BEFORESKIP : Absolute value = skip to leave above the heading.  
%                 If negative, then paragraph indent of text following 
%                 heading is suppressed.
%    AFTERSKIP  : if positive, then skip to leave below heading,
%                       else - skip to leave to right of run-in heading.
%    STYLE      : commands to set style
%  If '*' missing, then increments the counter.  If it is present, then
%  there should be no [ALTHEADING] argument.  A sectioning command
%  is normally defined to \@startsection + its first six arguments.
\makeatother

% Colors
\definecolor{darkgreen}{rgb}{0.01, 0.75, 0.24}
\definecolor{darkcyan}{rgb}{0.0, 0.55, 0.55}
\definecolor{mycolor}{rgb}{0.01, 0.75, 0.24}
\definecolor{takeawaycolor}{rgb}{0.75, 0, 0}
\definecolor{mygray}{gray}{0.9}
\definecolor{myred}{rgb}{0.75, 0, 0}
\definecolor{alg1}{rgb}{0.898, 1, 0.914}
\definecolor{alg2}{rgb}{0.925, 0.988, 1}
\definecolor{alg3}{rgb}{1, 1, 0.906}
\definecolor{alg4}{rgb}{1, 0.922, 0.922}
% hypen
\mathchardef\hyphen="2D

% Formal
\newtheoremstyle{sltheorem}
{}                % Space above
{}                % Space below
{\slshape}        % Theorem body font % (default is "\upshape")
{}                % Indent amount
{\bfseries}       % Theorem head font % (default is \mdseries)
{.}               % Punctuation after theorem head % default: no punctuation
{ }               % Space after theorem head
{}                % Theorem head spec
\theoremstyle{sltheorem}
% \theoremstyle{plain}
\newtheorem{prop}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
\newtheorem{observation}{Observation}
\newtheorem{condition}{Condition}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{Lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{property}{Property}
\newtheorem{heuristic}{Heuristic}

\newmdenv[
  backgroundcolor=gray!20,
  linecolor=gray,
  linewidth=1pt,
  roundcorner=5pt,
  skipabove=6pt,
  skipbelow=6pt,
  innertopmargin=1pt,
  innerbottommargin=4pt,
  innerleftmargin=6pt,   % tighter left margin inside the box
  innerrightmargin=6pt   % tighter right margin inside the box
]{graybox}


% For custom bold heading
\newcommand{\myitem}[1]{\vspace{1mm}\noindent\textbf{#1}}
\newcommand{\myitemit}[1]{\noindent\textit{#1}}
% \makeatletter\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}{3.25ex \@plus1ex \@minus.2ex}{-1em}{\normalfont\normalsize\itshape}}\makeatother

\newcommand{\remove}[1]{}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

% Some shortcuts for text
\newcommand{\first}{\emph{(i)}\xspace}
\newcommand{\second}{\emph{(ii)}\xspace}
\newcommand{\third}{\emph{(iii)}\xspace}
\newcommand{\fourth}{\emph{(iv)}\xspace}
\newcommand{\fifth}{\emph{(v)}\xspace}
\newcommand{\sixth}{\emph{(vi)}\xspace}
\newcommand{\seventh}{\emph{(vii)}\xspace}
\usepackage{xcolor}
\definecolor{light-gray}{gray}{0.9}
\usepackage{tcolorbox}
% \usepackage{soul}
% \newcommand{\mathcolorbox}[2]{\colorbox{#1}{$\displaystyle #2$}}


\newcommand{\First}{\emph{(I)}\xspace}
\newcommand{\Second}{\emph{(II)}\xspace}
\newcommand{\Third}{\emph{(III)}\xspace}
\newcommand{\Fourth}{\emph{(IV)}\xspace}
\newcommand{\Fifth}{\emph{(V)}\xspace}
\newcommand{\Sixth}{\emph{(VI)}\xspace}
\newcommand{\Seventh}{\emph{(VII)}\xspace}

\newcommand{\ie}{i.e., \@}
\newcommand{\eg}{e.g., \@}
\newcommand{\etc}{etc., \@}
\newcommand{\etal}{et al.\xspace}

\newcommand{\xref}[1]{\S\ref{#1}}
\newcommand{\axref}[1]{Appendix~\ref{#1}}
\newcommand{\cref}[1]{Chapter~\ref{#1}}
\newcommand{\pxref}[1]{(\xref{#1})}
\newcommand{\fref}[1]{Fig.~\ref{#1}}
\newcommand{\tref}[1]{Table~\ref{#1}}
